Fair Machine Guidance to Enhance Fair Decision Making in Biased People

Teaching unbiased decision-making is crucial for addressing biased decision-making in daily life. Although both raising awareness of personal biases and providing guidance on unbiased decision-making are essential, the latter topics remains under-researched. In this study, we developed and evaluated an AI system aimed at educating individuals on making unbiased decisions using fairness-aware machine learning. In a between-subjects experimental design, 99 participants who were prone to bias performed personal assessment tasks. They were divided into two groups: a) those who received AI guidance for fair decision-making before the task and b) those who received no such guidance but were informed of their biases. The results suggest that although several participants doubted the fairness of the AI system, fair machine guidance prompted them to reassess their views regarding fairness, reflect on their biases, and modify their decision-making criteria. Our findings provide insights into the design of AI systems for guiding fair decision-making in humans.

==> source/body/code-distribution-hint.tex <==
\begin{table}[t]
    \centering
    \caption{Distribution of evaluation about machine advice for each condition (BF: Bias feedback, FMT: Fair machine guidance) and group (W: Worse, B: Better, R: Reverse). A hyphen indicates $0\%$.}
\begin{tabular}{|p{4.8cm}|rrr|rrr|rrr|rr|}
\hline
\multirow{3}{*}{} & \multicolumn{6}{c|}{Income} & \multicolumn{5}{c|}{Credit} \\ \cline{2-12} 
 & \multicolumn{3}{c|}{BF} & \multicolumn{3}{c|}{FMT} & \multicolumn{3}{c|}{BF} & \multicolumn{2}{c|}{FMT} \\ \cline{2-12} 
 & \multicolumn{1}{c}{W} & \multicolumn{1}{c}{B} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c}{W} & \multicolumn{1}{c}{B} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c}{W} & \multicolumn{1}{c}{B} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c}{B} & \multicolumn{1}{c|}{R} \\ \hline
Incorrect & - & - & \multicolumn{1}{r|}{-} & - & - & - & - & - & \multicolumn{1}{r|}{-} & 7\% & - \\ \hline
Confusing & - & - & \multicolumn{1}{r|}{-} & - & - & - & - & 13\% & \multicolumn{1}{r|}{-} & 7\% & - \\ \hline
Unfair & - & 5\% & \multicolumn{1}{r|}{-} & - & - & 17\% & - & - & \multicolumn{1}{r|}{29\%} & - & 33\% \\ \hline
Fair & 13\% & 24\% & \multicolumn{1}{r|}{25\%} & 14\% & 25\% & - & 50\% & 38\% & \multicolumn{1}{r|}{29\%} & 50\% & 50\% \\ \hline
Broad in perspective & - & - & \multicolumn{1}{r|}{-} & 14\% & 13\% & - & - & - & \multicolumn{1}{r|}{-} & - & - \\ \hline
Inconsistent & - & - & \multicolumn{1}{r|}{-} & 14\% & - & 17\% & - & - & \multicolumn{1}{r|}{-} & 14\% & - \\ \hline
Partially helpful & - & - & \multicolumn{1}{r|}{-} & - & - & - & - & - & \multicolumn{1}{r|}{-} & - & - \\ \hline
Partially understandable & - & - & \multicolumn{1}{r|}{-} & - & 13\% & - & - & - & \multicolumn{1}{r|}{-} & 7\% & - \\ \hline
Partially convincing & - & - & \multicolumn{1}{r|}{13\%} & 14\% & 25\% & 33\% & - & - & \multicolumn{1}{r|}{-} & 7\% & 17\% \\ \hline
Unfair about the other sensitive attributes than race (gender) & - & - & \multicolumn{1}{r|}{-} & 14\% & - & 17\% & - & - & \multicolumn{1}{r|}{-} & - & 50\% \\ \hline
Don't know how to use & 13\% & 5\% & \multicolumn{1}{r|}{-} & - & - & - & - & - & \multicolumn{1}{r|}{-} & - & - \\ \hline
Suspicious about the decision criteria & - & - & \multicolumn{1}{r|}{-} & 43\% & - & - & - & - & \multicolumn{1}{r|}{-} & 36\% & 67\% \\ \hline
Not helpful & - & - & \multicolumn{1}{r|}{-} & - & - & - & - & 25\% & \multicolumn{1}{r|}{-} & - & - \\ \hline
Objective & - & - & \multicolumn{1}{r|}{-} & 29\% & - & - & - & 25\% & \multicolumn{1}{r|}{-} & 21\% & 33\% \\ \hline
Advice given in numbers is easy to understand & - & - & \multicolumn{1}{r|}{-} & - & - & - & - & - & \multicolumn{1}{r|}{29\%} & - & - \\ \hline
Suspicious about the number & 25\% & 33\% & \multicolumn{1}{r|}{56\%} & 14\% & - & - & - & 38\% & \multicolumn{1}{r|}{43\%} & 7\% & - \\ \hline
Suspicious about the final decision & - & - & \multicolumn{1}{r|}{-} & 29\% & 13\% & 17\% & - & - & \multicolumn{1}{r|}{-} & - & 50\% \\ \hline
Unclear reasoning & - & - & \multicolumn{1}{r|}{-} & - & 25\% & 17\% & - & - & \multicolumn{1}{r|}{-} & 21\% & 50\% \\ \hline
Based on simple criteria & - & - & \multicolumn{1}{r|}{-} & 14\% & - & - & - & - & \multicolumn{1}{r|}{-} & - & - \\ \hline
Correct and convincing & - & 14\% & \multicolumn{1}{r|}{6\%} & 14\% & 50\% & 50\% & - & - & \multicolumn{1}{r|}{14\%} & 14\% & - \\ \hline
Understandable & - & - & \multicolumn{1}{r|}{-} & - & - & 17\% & - & - & \multicolumn{1}{r|}{-} & 7\% & 17\% \\ \hline
Not understandable & 38\% & 5\% & \multicolumn{1}{r|}{-} & - & - & - & 50\% & - & \multicolumn{1}{r|}{-} & 14\% & - \\ \hline
Confusing because advice is different from my criteria & - & - & \multicolumn{1}{r|}{-} & 14\% & - & - & - & - & \multicolumn{1}{r|}{-} & 7\% & - \\ \hline
Aligned with my criteria & - & - & \multicolumn{1}{r|}{-} & 14\% & - & - & - & - & \multicolumn{1}{r|}{-} & 7\% & - \\ \hline
Differed from my criteria & - & - & \multicolumn{1}{r|}{-} & - & 13\% & - & - & - & \multicolumn{1}{r|}{-} & - & - \\ \hline
Helpful to check the correctness of my own judgements & - & - & \multicolumn{1}{r|}{6\%} & 14\% & - & - & - & - & \multicolumn{1}{r|}{-} & - & - \\ \hline
Identified my mistakes and biases & - & 19\% & \multicolumn{1}{r|}{6\%} & - & 25\% & 17\% & - & - & \multicolumn{1}{r|}{-} & 21\% & - \\ \hline
\end{tabular}\label{tb:5-2-hint}
\end{table}


==> source/body/code-distribution-strategy.tex <==
\begin{table}[t]
    \centering
    \caption{Distribution of strategies for each condition (BF: Bias feedback, FMT: Fair machine guidance) and group (W: Worse, B: Better, R: Reverse). A hyphen indicates $0\%$.}
\begin{tabular}{|p{4.8cm}|rrr|rrr|rrr|rr|}
\hline
& \multicolumn{6}{c|}{Income}                                                                                                                    & \multicolumn{5}{c|}{Credit}                                                                                                                    \\ \cline{2-12} 
& \multicolumn{3}{c|}{BF}                                                & \multicolumn{3}{c|}{FMT}                                               & \multicolumn{3}{c|}{BF}                                                & \multicolumn{2}{c|}{FMT}                                               \\ \cline{2-12} 
& \multicolumn{1}{c}{W} & \multicolumn{1}{c}{B} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c}{W} & \multicolumn{1}{c}{B} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c}{W} & \multicolumn{1}{c}{B} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c}{B} & \multicolumn{1}{c|}{R} \\ \hline
Adjusted the number by race (gender)                                                        & 50\%                  & 29\%                  & 38\%                  & 29\%                  & -                   & -                    & -                   & -                   & 29\%                  & -                   & 17\%                  \\ \hline
Judged without looking at race (gender)                                                                   & -                   & 29\%                  & 50\%                  & 14\%                  & 25\%                  & 33\%                   & 50\%                  & 25\%                  & 43\%                  & 7\%                   & 17\%                  \\ \hline
Balanced the teacher's criteria with my criteria& -                   & 10\%                  & -                   & -                   & 25\%                  & 33\%                   & -                   & -                   & -                   & -                   & -                   \\ \hline
Followed the advice and adjusted my criteria         & 25\%                  & 14\%                  & 13\%                  & 29\%                  & 50\%                  & 17\%                   & 100\%                 & 38\%                  & 14\%                  & 43\%                  & 67\%                  \\ \hline
Judged based on a lot of information                                                            & 13\%                  & -                   & -                   & -                   & -                   & -                    & -                   & 13\%                  & -                   & -                   & -                   \\ \hline
Followed my own criteria                                                                        & 13\%                  & 10\%                  & 19\%                  & -                   & 13\%                  & -                    & -                   & 13\%                  & -                   & 14\%                  & 17\%                  \\ \hline
Judged objectively and logically                                                                & -                   & -                   & -                   & 14\%                  & -                   & -                    & 50\%                  & 13\%                  & 14\%                  & 7\%                   & 33\%                  \\ \hline
\end{tabular}
\label{tb:5-1-senryaku}
\end{table}

